Stellar Rotation in the K2 Sample: Evidence for Modified Spindown

We analyze light curves of 284,834 unique K2 targets using a Gaussian process model with a quasi-periodic kernel function. By crossmatching K2 stars to observations from Gaia Data Release 2, we have identified 69,627 likely main-sequence stars. From these we select a subsample of 8,977 stars on the main-sequence with highly precise rotation period measurements. With this sample we recover the gap in the rotation period-color diagram first reported by \cite{McQuillan2013}. While the gap was tentatively detected in \cite{Reinhold2020}, this work represents the first robust detection of the gap in K2 data for field stars. This is significant because K2 observed along many lines of sight at wide angular separation, in contrast to Kepler's single line of sight. Together with recent results for rotation in open clusters, we interpret this gap as evidence for a departure from the $t^{-1/2}$ Skumanich spin down law, rather than an indication of a bimodal star formation history. We provide maximum likelihood estimates and uncertainties for all parameters of the quasi-periodic light curve model for each of the 284,834 stars in our sample.

==> mapping.tex <==
\section{Mapping Galactic Structure with Stellar Rotation}\label{sec:structure}

    While there is still much that is poorly 
    understood regarding the relationship between 
    stellar rotation and age, the fact that 
    stars lose angular momentum over their 
    main sequence lifetimes is well-established. 
    Thus while gyrochronology does not 
    yet allow us to precisely determine stellar 
    ages, it does allow us to probe the 
    relative ages of stellar populations. K2's 
    many lines of sight offer us a unique 
    opportunity to explore this aspect of 
    galactic structure in the nearby galaxy. 
    
    Care must be taken to choose appropriate 
    metrics for this work. It may be tempting 
    to simply measure the mean or median 
    rotation period for stars binned by 
    their galactocentric position, but there 
    are problems with this approach. First, 
    we need to correct for the fact that 
    stars of different spectral types 
    spin down at different rates. We would 
    typically do this by subtracting a 
    theoretical gyrochrone from the 
    rotation periods. However, recent 
    work \citep{} has shown that current 
    gyrochronological models are unreliable and 
    that rotation periods remain nearly constant 
    for stars of some spectral types over 
    periods of hundreds of millions of years \citep{}.
    As a result we advise against using 
    theoretical gyrochrones to determine the 
    relative ages of field stars. 
    
    A second problem is that the stars in each 
    positional bin may potentially be drawn 
    from many different sub-populations, 
    each having a distinct age distribution. 
    The thin disk itself is a superposition 
    of populations with ages ranging from 
    0-10 Gyrs \citep{Sharma2019}. It is 
    therefore unjustified to assume Gaussian 
    age distribution within an individual 
    positional bin as we implicitly 
    do when we use the mean rotation 
    period as an estimator of the age of 
    the population. Even assuming unimodality 
    may be unjustified for stars 
    in the thin disk, suggesting that the 
    median would be a poor estimator as well. 
    
    %----------- fix next paragraph and down 
    
    To avoid these problems we group stars 
    into two categories by their rotation period: 
    ``old stars'' are those with rotation periods 
    that place them above the gap in Figure 
    \ref{fig:period_color} and ``young stars'' 
    are those below the gap. To uncover 
    galactic structure in the K2 sample we 
    consider the ratio between the number of 
    stars in each population, 
    $N_\mathrm{young}/N_\mathrm{old}$. This 
    parameter does not depend upon theoretical 
    isochrones or on assumptions about 
    the shape of the rotation period distribution 
    other than the presence of the gap, and 
    it should be less sensitive to the K2 selection 
    function as well. We consider 
    stars above the gap (``old'' stars) to be those 
    with rotation periods satisfying:
    \begin{equation}
        \label{eqn:old}
        P_\mathrm{rot} > 12(M_B-M_V)^{1.8}
    \end{equation}
    and stars below the gap are those with 
    \begin{equation}
        \label{eqn:young}
        P_\mathrm{rot} < 12(M_B-M_V)^{1.8}
    \end{equation}
    where the coefficient and exponent in 
    equations \ref{eqn:old} and \ref{eqn:young} 
    are chosen by eye to match the position 
    and trend of the gap log period-color space. 
    In assigning the labels ``old'' and ``young'' 
    to the two populations we assume that 
    a star, having spun down across the gap, 
    does not ever return to the population 
    below the gap. 
    
    $N_\mathrm{young}/N_\mathrm{old}$ measures the 
    relative dominance of the population of 
    young stars over that of older stars in 
    a given positional bin. 
    Figure \ref{fig:balance_z} shows a 
    map of this ratio in $R_\mathrm{xy}$ vs. $z$ space. 
    Here $z$ represents the distance of the stars from 
    the galactic mid-plane irrespective of direction 
    (above or below the plane). Because the map 
    appears to be symmetric with respect to the 
    sign of $z$, we take the absolute value 
    of this coordinate in order to increase 
    the sample size in the bins at large $z$. 
    
    \begin{figure*}
	    \plotone{figures/balance_z.pdf}
	    \caption{Right: A spatially resolved 
	    map of $\log(N_\mathrm{young}/N_\mathrm{old}$ 
	    demonstrating that the population of ``old'' stars 
	    (those with rotation periods longer than the gap) 
	    is more dominant at higher distances from the 
	    galactic plane. Left: The $R_{xy}$ integrated 
	    $N_\mathrm{young}/N_\mathrm{old}$ as a function of 
	    $z$. The bars are colored by the mean of 
	    $\log(N_\mathrm{young}/N_\mathrm{old})$ and the 
	    size of the bars indicates $N_\mathrm{young}/N_\mathrm{old}$. 
	    Note the exponential decay in the profile shown 
	    in the left panel.}
	    \label{fig:balance_z}
	\end{figure*}
    
    The most prominent feature of this map is the 
    gradient in the $z$ direction moving from a 
    larger population of young stars near $z=0$ 
    towards a larger population of old stars in 
    the highest $z$ bins. The total number 
    of stars with well-determined rotation 
    periods decreases at larger $z$, and beyond 
    about $z=400$ pc there are not enough stars to 
    measure the ratio of populations accurately. 
    
    The left panel of Figure \ref{fig:balance_z} 
    shows the exponential decay in 
    $N_\mathrm{young}/N_\mathrm{old}$ as a function 
    of height $z$. The thick disk is a population of low 
    metallicity and high $[\alpha/\mathrm{Fe}]$ 
    stars centered on the plane of the milky way 
    \citep{Carillo2020}. It has a scale height of 
    about 900 pc relative to the thin disk's 
    scale height of about 300 pc \citep{Juric2008}. 
    The low metallicity of the thick disk 
    points to an older population of star. This 
    conclusion is supported by isochrone fitting 
    of thick disk globular clusters \citep{Liu2000}, 
    observations of ultracool white dwarfs 
    in the thick disk \citep{Gianninas2015}, and 
    asteroseismology \citep{Sharma2019},
    all of which give an age of greater than 10 Gyr. 
    
    In contrast, the thin disk is the result of 
    ongoing star formation in the plane of the 
    galaxy, having a number of distinct 
    populations ranging in age from 0-10 
    Gyrs \citep{Sharma2019}. It is therefore 
    likely that we have included some portion 
    of thin disk stars in our ``old'' stars 
    sample, but have been more successful in 
    excluding thick disk stars from our 
    ``young'' stars sample since stars in the 
    thick disc should be far too old to have 
    rotation periods that place them below 
    the period gap in Figure \ref{fig:period_color}. 
    
    If we assume a number density profile 
    for the thick and thin disks, we can 
    compute the expected scaling of 
    $N_\mathrm{young}/N_\mathrm{old}$ with 
    height. We take the density distributions 
    of the two disk populations from 
    \cite{Juric2008}, who gives the 
    profile of both disks as:
    \begin{equation}
        \rho_D(Z) \propto \mathrm{exp}\left(-\frac{Z+Z_\odot}{H_i}\right)
    \end{equation}
    where we have ignored the radial dependence 
    of the profile. The thin disk profile 
    is found by taking $H_1 = 300$ pc and 
    the thick disk is has $H_2=900$ pc \citep{Juric2008}. 
    Taking the ratio between the two density profiles 
    we have
    \begin{eqnarray}
        \frac{N_\mathrm{young}(Z)}{N_\mathrm{old}(Z)} = \frac{\rho_1(Z)}{\rho_2(Z)} &\propto& 
            \mathrm{exp}\left(\frac{Z+Z_\odot}{H_2} - \frac{Z+Z_\odot}{H_1}\right) \\
            &\propto& \mathrm{exp}\left((Z+Z_\odot)\frac{H_1-H_2}{H_1H_2}\right)
    \end{eqnarray}
    For the values of $H_1$ and $H_2$ given above 
    we find 
    \begin{eqnarray}
        \frac{N_\mathrm{young}(Z)}{N_\mathrm{old}(Z)} &\propto& e^{-(Z+Z_\odot)/450\mathrm{ pc}} \\
        &\propto& e^{Z/\mathrm{450 pc}}
    \end{eqnarray}
    
    Before comparing this exponential decay 
    to the profile in Figure \ref{fig:balance_z}, 
    we should outline several caveats. First, 
    we do not expect that $N_\mathrm{thin}/N_\mathrm{thick}$ 
    will be exactly equal to $N_\mathrm{young}/N_\mathrm{old}$. 
    Because the thin disk contains stellar populations 
    as old as 10 Gyr, we will end up including  
    stars from the older end of the thin disk 
    age range in $N_\mathrm{old}$. Additionally, 
    we only have estimates of the ratio out 
    to about $400$ pc, which is less than one 
    scale-height. This makes reliable inference of 
    the scale-height difficult. 
    
    We fit a function of the form
    \begin{equation}
        y = Ae^{x/L}
    \end{equation}
    to the $R_{xy}$-summed values 
    of $N_\mathrm{young}/N_\mathrm{old}$ 
    shown in the left-hand panel of Figure \ref{fig:balance_z} 
    and find the scale-height of the 
    exponential decay to be $346^{\pm20}$ pc.
    
    Given that we don't expect the ratio 
    of populations to correspond 
    exactly to the ratio of stellar densities in 
    the thin and thick disks, we consider this 
    measurement to be very uncertain. The 
    $\pm$ 20 pc error bars are almost 
    certaintly an under-estimate of the 
    true error since we didn't take into 
    account the uncertainty from counting 
    stars in each bin to compute 
    $N_\mathrm{young}/N_\mathrm{old}$. Furthermore, 
    since we have only measured periods less than 
    30 days, we are biased against slow rotating, 
    and thus older, stars. This bias should 
    decrease our inferred scale hepreviight since 
    it reduces the population of old stars and 
    therefore steepens the ratio 
    $N_\mathrm{young}/N_\mathrm{old}$.
    Despite these issues, the scale height 
    we find here does agree in magnitude
    with the expected value of 450 pc, which 
    we take as tentative confirmation that 
    we are indeed measuring galactic structure 
    from stellar rotation alone. 
    
    
    \cite{McQuillan2014} and \cite{Davenport2018} 
	propose that the gap is an artifact of 
	a recent ($< 500$ Myr) burst of star formation 
	producing a population of young stars which 
	make up the fast-rotating sequence below the 
	gap. The single pointing of the Kepler mission, 
	on which both of these analyses relied, admits 
	the possibility of a local burst of star formation 
	in the direction of the Kepler field accounting 
	for the fast-rotating population. We have shown 
	that the gap exists in all K2 Campaigns at 
	the same location and with the same width. 
	While these facts don't rule out the possibility 
	that the gap is related to star formation history, 
	it does place strong constraints on that star 
	formation history. The burst would have to 
	be isotropic in the solar neighborhood. 
	The sharp edges of the gap and the upward 
	concavity of the fast-rotating sequence both 
	pose challenges for models of this burst. 
	\cite{vanSaders2019} simulated bursty 
	star formation in the TRILEGAL simulation 
	and was able to approximately reproduct the 
	bimodality, but noted that the shape of the 
	gap as seen in Kepler was not reproduced 
	successfuly. The additional details of the 
	shape of the gap presented here will only 
	make it more difficult to reproduce the gap 
	using star formation simulations.
